The CLASS Quasar Catalog: Coronal Line Activity in Type 1 SDSS Quasars

We conduct the first systematic survey of a total of eleven optical coronal lines in the spectra of a large sample of low redshift (z < 0.8) Type 1 quasars observed by the Sloan Digital Sky Survey (SDSS). We find that strong coronal line emission is rare in SDSS even in Type 1 quasars; only 885 out of 19,508 (4.5%) galaxies show at least one coronal line, with higher ionization potential lines ($>100$eV) being even rarer. The [Ne V] $\lambda$3426 line, which constitutes the majority of detections, is strongly correlated with the bolometric luminosity. These findings suggest that the optical coronal lines are significantly suppressed in the majority of local AGNs, possibly as a result of the presence of dust in the emitting regions. We find that the incidence of ionized outflows is significantly higher in coronal line emitters compared with non-coronal line emitters, possibly suggesting that dust destruction in outflows enhances coronal line emission in AGNs. Many coronal lines show line profiles that are broader than those of narrow lines, and are blue-shifted relative the lower ionization potential lines, suggesting outflows in the highly ionized gas. Given the limited number of detections, we do not find any statistically significant trends of detection statistics, or line ratios with black hole mass, Eddington ratio, or AGN bolometric luminosity. The catalog is publicly available and can provide a useful database of the coronal line properties of low redshift quasars that can be compared to the growing number of high-z AGNs discovered by JWST.

==> tables/line_table_full.tex <==
\startlongtable
\begin{deluxetable*}{ccccccccccccc}
\tabletypesize{\footnotesize}
\tablecaption{Optical coronal emission lines from 3346--7892 \AA. $\lambda_{\rm rest}$ is the rest wavelength, $\rho_{\rm crit}$is the critical density, $L$ is the luminosity, FWHM is the full-width at half-maximum of theline profile, $v_{\rm off}$ is the velocity offset relative to the stellar velocity, and $N$ is the number of detections.For $L$, FWHM, and $v_{\rm off}$, the values shown are (mean) $\pm$ (standard deviation).}
\tablehead{\colhead{Line} & \colhead{$\lambda_{\rm rest}$}\textsuperscript{1} & \colhead{$\rho_{\rm crit}$} & \colhead{IP}\textsuperscript{2} & \colhead{Transition} & \colhead{$L_{Thresh}$} & \colhead{$L$} & \colhead{FWHM} & \colhead{$v_{\rm off}$} & \colhead{EW} & \colhead{Detections}\textsuperscript{3} & \colhead{Detections}\textsuperscript{3} & \colhead{$N$}\\
\colhead{} & \colhead{(\AA)} & \colhead{(cm$^{-3}$)} & \colhead{(eV)} & \colhead{} & \colhead{(log(erg s$^{-1})$)} & \colhead{(log(erg s$^{-1})$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(\AA)} & \colhead{(\%)} & \colhead{(\%)} & \colhead{}}
\decimals
\startdata
\lbrack \ion{Fe}{11}\rbrack & 7891.800 & $6.39 \times 10^8$ & 262.10 & $^3$P$_2 - ^3$P$_1$ & 40.07 & $40.68 \pm 0.00$ & $282 \pm 0$ & $-6 \pm 0$ & $1.60 \pm 0.00$ & ${0.22}^{+0.51}_{-0.18}$ & ${0.22}^{+0.51}_{-0.18}$ & 1 \\
\lbrack \ion{S}{12}\rbrack & 7611.000 & $7.09 \times 10^9$ & 504.78 & $^2$P$^0_{1/2} - ^2$P$^0_{3/2}$ & 40.21 & --- & --- & --- & --- & --- & --- & 0 \\
\lbrack \ion{Fe}{10}\rbrack & 6374.510 & $4.45 \times 10^8$ & 235.04 & $^2$P$^0_{3/2} - ^2$P$^0_{1/2}$ & 40.43 & $40.73 \pm 0.21$ & $646 \pm 247$ & $-25 \pm 86$ & $2.13 \pm 0.62$ & ${0.157}^{+0.084}_{-0.058}$ & ${0.114}^{+0.061}_{-0.042}$ & 7 \\
\lbrack \ion{Fe}{7}\rbrack & 6087.000 & $4.46 \times 10^7$ & 99.00 & $^3$F$_3 - ^1$D$_2$ & 40.49 & $40.93 \pm 0.29$ & $617 \pm 208$ & $-50 \pm 117$ & $2.23 \pm 1.04$ & ${1.34}^{+0.18}_{-0.16}$ & ${0.835}^{+0.110}_{-0.098}$ & 71 \\
\lbrack \ion{Fe}{7}\rbrack & 5720.700 & $3.72 \times 10^7$ & 99.00 & $^3$F$_2 - ^1$D$_2$ & 40.61 & $40.76 \pm 0.19$ & $547 \pm 194$ & $-31 \pm 114$ & $1.94 \pm 0.66$ & ${0.181}^{+0.062}_{-0.048}$ & ${0.135}^{+0.046}_{-0.035}$ & 14 \\
\lbrack \ion{Fe}{5}\rbrack & 3891.280 & $1.61 \times 10^8$ & 54.80 & $^5$D$_4 - ^3$F2$_4$ & 40.69 & $40.88 \pm 0.00$ & $1038 \pm 0$ & $90 \pm 0$ & $2.12 \pm 0.00$ & ${0.0054}^{+0.0124}_{-0.0045}$ & ${0.0054}^{+0.0124}_{-0.0045}$ & 1 \\
\lbrack \ion{Fe}{5}\rbrack & 3839.270 & $1.00 \times 10^8$ & 54.80 & $^5$D$_3 - ^3$F2$_3$ & 40.64 & --- & --- & --- & --- & --- & --- & 0 \\
\lbrack \ion{Fe}{7}\rbrack & 3758.920 & $4.02 \times 10^7$ & 99.00 & $^3$F$_4 - ^1$G$_4$ & 40.81 & $41.95 \pm 0.42$ & $840 \pm 341$ & $37 \pm 243$ & $4.12 \pm 4.27$ & ${0.022}^{+0.017}_{-0.010}$ & ${0.021}^{+0.017}_{-0.010}$ & 4 \\
\lbrack \ion{Ne}{5}\rbrack & 3425.881 & $1.90 \times 10^7$ & 97.11 & $^3$P$_2 - ^1$D$_2$ & 40.62 & $41.88 \pm 0.37$ & $787 \pm 274$ & $-107 \pm 115$ & $4.64 \pm 4.17$ & ${5.39}^{+0.19}_{-0.18}$ & ${4.49}^{+0.16}_{-0.15}$ & 847 \\
\lbrack \ion{Ne}{5}\rbrack & 3345.821 & $1.14 \times 10^7$ & 97.11 & $^3$P$_1 - ^1$D$_2$ & 40.64 & $41.67 \pm 0.31$ & $665 \pm 196$ & $-77 \pm 103$ & $4.38 \pm 3.78$ & ${0.400}^{+0.113}_{-0.090}$ & ${0.153}^{+0.044}_{-0.035}$ & 19 \\
\lbrack \ion{Ne}{4}\rbrack & 2424.403 & TODO & 63.42 & TODO & 41.09 & $42.47 \pm 0.22$ & $893 \pm 238$ & $-348 \pm 101$ & $1.45 \pm 0.43$ & ${0.128}^{+0.054}_{-0.040}$ & ${0.125}^{+0.053}_{-0.039}$ & 10 \\
\enddata
\begin{tablenotes}
	\item[0] \textsuperscript{1}Wavelengths taken from: \url{https://physics.nist.gov/PhysRefData/ASD/lines_form.html}.
	\item[1] \textsuperscript{2}Ionization potential taken from: \url{https://physics.nist.gov/PhysRefData/ASD/ionEnergy.html}.
	\item[2] \textsuperscript{3}The detection percentage columns are calculated as the number N over the total number of spectra that \
          could have detected the line. The denominator of the left detection column is determined by the number \
          of galaxies whose luminosity threshold exceeds 3 times the average CL luminosity and the right is determined \
          with respect to 3 times the maximum CL luminosity. In both cases, the errors are 68\% confidence intervals \
          calculated with binomial statistics.
\end{tablenotes}
\label{tab:lines}
\end{deluxetable*}

